MP5: A Multi-modal Open-ended Embodied System in Minecraft via Active Perception

It is a long-lasting goal to design an embodied system that can solve long-horizon open-world tasks in human-like ways. However, existing approaches usually struggle with compound difficulties caused by the logic-aware decomposition and context-aware execution of these tasks. To this end, we introduce MP5, an open-ended multimodal embodied system built upon the challenging Minecraft simulator, which can decompose feasible sub-objectives, design sophisticated situation-aware plans, and perform embodied action control, with frequent communication with a goal-conditioned active perception scheme. Specifically, MP5 is developed on top of recent advances in Multimodal Large Language Models (MLLMs), and the system is modulated into functional modules that can be scheduled and collaborated to ultimately solve pre-defined context- and process-dependent tasks. Extensive experiments prove that MP5 can achieve a 22% success rate on difficult process-dependent tasks and a 91% success rate on tasks that heavily depend on the context. Moreover, MP5 exhibits a remarkable ability to address many open-ended tasks that are entirely novel.

==> sec/3_method.tex <==
\section{Method}
\label{sec:Method}
In this section, we define and introduce two metrics for measuring the difficulty of open tasks in an open world in Section~\ref{sec:Difficulty}. Following this, we provide a detailed explanation of the overall architecture and constituent modules of TACTICIAN in Section~\ref{TACTICIAN Architecture}. Finally, we describe the process of active perception and the construction of the MineLLM in Section~\ref{Active Perception}.


\subsection{The Temporal and Spatial Difficulty of Task}
\label{sec:Difficulty}

Compared to the relatively simple scenarios of robotic arms, open tasks in open environments not only require more abstract levels of reasoning processes, accomplished by completing sequential subtasks to finish the final task, but the perceptual information required to complete each subtask also differs. This leads to a significant performance drop when traditional methods are adapted to complete open tasks in open environments.

% To address these challenges, we first deconstructed the corresponding embodied tasks from various aspects. We believe that if the completion of a task requires new tools or skills, then gaining new tools or skills becomes a prerequisite, constituting a reasoning step. Similarly, if completing a task requires more than one type of information, acquiring an additional category of perceptual information becomes a requirement, constituting a perceptual step. Based on our definitions of reasoning steps and perceptual steps, we defined two difficulty standards for open tasks in an open world:

To address these challenges, we first deconstructed the corresponding embodied tasks from various aspects. We believe that if the completion of a task requires new tools or skills, then gaining new tools or skills becomes a prerequisite, constituting a reasoning step. Every reasoning step need a period of time to be a accomplished.
On the contrary, scene understanding and perception conduct only at a moment in time, if completing a task requires more than one type of information, acquiring an additional category of perceptual information becomes a requirement, constituting a perceptual step. Based on our definitions of reasoning steps and perceptual steps, we defined two difficulty standards for open tasks in an open world:

\textbf{Temporal Difficulty}: The total reasoning steps needed to accomplish the task.

\textbf{Spatial Difficulty}: The total amount of perceptual information required to accomplish the task.

In the Minecraft simulation platform, crafting a diamond pickaxe requires multiple reasoning steps, the agent first needs to make wood picks, stone picks, iron picks and other necessary tools thus it is a task of high temporal difficulty. In contrast, locating a pig under a tree in a plain requires various perceptual information to complete the task, the agent needs to judge whether the scene has pigs, trees and their relationship, and at the same time ensure that it is located in the plain ecological environment at the current moment, hence it is a task of high spatial difficulty. From these examples, it's easy to see that tasks with high temporal and high spatial difficulties can be integrated, resulting in evidently more challenging tasks (for instance, using a diamond pickaxe to kill a pig on a plain). In this paper, considering the cost of model reasoning and time, we discuss and experiment with the two types of difficulty indicators separately. The specific task settings are referred to in the experimental section.

\subsection{TACTICIAN Architecture}
\label{TACTICIAN Architecture}

\begin{figure*}
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=1\linewidth]{figure/Active perception.png}
\end{center}
% \vspace{-3mm}
   \caption{A demonstration of the process of Activation Perception. The context in the figure is modified for better visualization. The full interaction dialogue of our agent is listed in Appendix XXX.}
\label{fig:Active perception}
\end{figure*}

As shown in Figure~\ref{fig:pipeline}, our agent is composed of five modules: the Decomposer for task decomposition, the Percipient for active perception, the Planner for planning and execution, the Checker for validation and feedback, and the External Memory for storing specialized knowledge and experiential knowledge.

We use a large language model as our zero-shot Decomposer. Given any instruction, the Decomposer can break down tasks of high temporal difficulty into a sequence of low temporal difficulty tasks and generate a subtask execution sequence, complete with manufacturing instructions based on the relevant professional knowledge stored in the External Memory. This sub-task sequence is provided to the Percipient and Plannerr. We use a trained multimodal large language model and a zero-shot large language model as our Percipient. Using the current subtask's description, the Percipient acquires the perceptual information needed for tasks of high spatial difficulty through active perception. After being validated by the Checker, agent will keep moving and looking until reaching a scene that satisfies all the perceived conditions or is already in a suitable scene to perform the subsequent behavior. 

We apply a large language model as our zero-shot Planner. The Planner uses the subtask information from the Decomposer, all the perceptual information including inventory content from the Percipient, the feedback from the last round of the Checker, and the practice memory from the External Memory to make a new round of workflow sequences after being checked by the Checker. In order to ensure that the basic units output by the Planner are purposeful rather than chaotic atomic action sequences, we define \textbf{Workflow}, a purposeful sequence composed of atomic actions (e.g., searching) that forms the minimum unit of the executable sequence deduced by the Planner. The definition of the Workflow not only adds purposefulness to the action sequence but also significantly reduces the pressure on the Planner. Following GITM\cite{zhu2023ghost}, we implement Workflow using hand-written scripts based on observations and basic operations interface provided by the MineDojo\cite{fan2022minedojo} simulator. The definition of relevant workflows can be seen in Table 1. 

Perceptual or decision-making errors often occur in real-world scenarios. We can't roll back to the moment before the decision was made like in game scenarios (such as Voyager\cite{wang2023voyager}) when setbacks or failures occur. Therefore, we specifically built a Checker centered around a large language model. It is responsible for checking whether the perceptual information provided by the Percipient is correct and sufficient, and whether the agent has completed the current subtask after executing the Planner's Workflow list. It provides feedback to the corresponding modules based on the inspection results, helping them correct the current information or execute the next subtask. 
More specifically, during the agent's execution phase, whenever an Active Perception ends, the Checker decides whether to continue executing the remaining Workflows in the list or continuely exploring and conduct next-term Active Perception based on the success or failure of the current-round Active Perception. 
When the agent finishes executing a workflow list, the checker will check whether the current subgoal is complete and gives feedback to proceed to the next subgoal or to replan the Workflow list of current subgoal. 
In addition, in more difficult scenarios, due to missing materials or errors in the subgoal list generated by the decomposer, the next subgoal cannot be planned. Checker will modify the next subgoal according to the current acquisition of items and skills and the description of the final task. This allows the agent to escape the endless loop of planning a subgoal that cannot be completed at the current stage.
Thanks to the Checker's real-time inspection capability, the agent can replan and eventually accomplish the task when in trouble. 

Compared to human decision-making processes, we set up an External Memory module, consisting of knowledge memory and practice memory. We believe that some physical laws or professional knowledge are hard for the agent to acquire through repetitive trials. Thus, we collected corresponding knowledge memory (e.g., ingredient ratios for tool production, distribution rules of different natural resources) from simulation platform documentation and Wikipedia for use by the Decomposer and Checker. Meanwhile, the practice memory stores examples of all successful tasks and some failed tasks, serving as a reference for the Planner.
\subsection{Active Perception}
\label{Active Perception}

Achieving tasks of high spatial difficulty requires more than just reasoning, therefore, we need a percipient that provides corresponding perceptual information according to task requirements. The Percipient achieves this through an active perception process which showed in Figure~\ref{Active Perception}. The large language model continuously feeds back perceptual needs based on existing perceptual information and task descriptions, and it communicates these needs to a multimodal large language model in the form of textual questions. The multimodal large language model understands the text and analyzes the corresponding perceptual results from real-time images obtained from the sensors. Through multiple rounds of communication between the large language model and the multimodal large language model, all the perceptual information needed to complete the current subtask is eventually obtained. We use a zero-shot large language model and collect data to train a multimodal large language model with perception, interaction, and analysis capabilities. 


\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figure/MLLM.png}
    \caption{The model architecture of MineLLM. Image is encoded by pre-trained vision encoder and decoded by LLM. Only the parameters of Alignment Net and LoRA are trainable.}
    \label{fig:mllm}
\vspace{-5mm}
\end{figure}


\textbf{Multimodal Perception Instruction Data.}
Human players perform actions in Minecraft mainly relying on their visual perception, without any cheating information in the simulation platform. We built multimodal instruction data in Minecraft scenario: the dataset contains 50K image data collected on the Minedojo\cite{fan2022minedojo} simulation platform, covering almost all Minecraft content, including various ecological environments, biological communities, different levels of brightness, underwater environments, etc., to ensure the model's ability to perceive the open world. On top of this, we collected, selected, and processed the corresponding perceptual information from the simulator that aligns with the image data (including the blocks in the field of view, creatures, weather, occupancy around the agent, etc. Notably, we specially processed and filtered the perspective information, retaining only the information that can be obtained visually). 
Based on the images and perceptual information, we constructed image-text question and answer pairs. To not limit the interaction form between the large language model and the multimodal large language model, and to make the interaction more flexible and robust, we designed templates for single-turn dialogue, multi-turn dialogues and caption. 
For each piece of perceptual information, we also designed multiple forms of questions and answers, greatly reducing the probability of interaction failure between the two models.
The total number of instruction data pair is 200K.

We plan to open-source all Multimodal Perception Instruction Data, hoping this dataset can facilitate other works and promote the development of the community. For detailed information on the dataset and data formats, please refer to the appendixXXX.

\textbf{MineLLM.} The overall framework of our MineLLM is depicted in Figure~\ref{fig:mllm}. Each training instance consists of an image and a multi-turn conversation data $(\boldsymbol{x}_1, \boldsymbol{y}_1, ..., \boldsymbol{x}_n, \boldsymbol{y}_n)$, where $\boldsymbol{x}_i$ and $\boldsymbol{y}_i$ are the human’s instruction and the system’s response at the $i$-th turn. Images are processed by vision encoder, whose feature are then projected to the same feature space as the text embeddings by a Alignment Net $f$. Instructions are directly tokenized by SentencePiece tokenizer\cite{kudo2018sentencepiece}, then the vision and text tokens are concatenated to feed into the LLM model. To finetune LLM efficiently, we add LoRA~\cite{hu2021lora} parameters $l$ to all projection layers in the self-attention layers. As shown in Figure~\ref{fig:mllm}, only Alignment Net and LoRA parameters are optimized during training. The training objective of MineLLM is defined as:
\begin{align}
    \mathcal{L}\left(\theta_{f}, \theta_{l}\right)=\prod_{i=1}^{n} p_{\theta}\left(\boldsymbol{y}_{i} \mid \boldsymbol{x}_{<i}, \boldsymbol{y}_{<i-1}, f\left(\mathcal{I}\right)\right)
\end{align}
where $\theta_{f}$ and $\theta_{l}$ correspond to the learnable parameters of the Alignment Net and LoRA. The $\mathcal{I}$ is the image representation produced by the vision encoder. More training setting could be found in the Implementation Details of Section~\ref{sec:Experimental Setup}.





% The overall framework of OEA consists of three main components: the Decomposer, the Perceptor, and the Planner. The Decomposer is responsible for analyzing and decomposing complex tasks. The Perceptor receives environmental information captured by sensors and can actively perceive based on the task at hand. Lastly, the Planner continuously interacts with the Perceptor to obtain sufficient perceptual information. Using this perceptual information, feedback, and memory, the Planner infers executable workflow sequences.

% \subsection{Decomposer}
% For conventional fixed tasks within fixed scenarios, people often assign a specific task to an embodied agent. These tasks can either be relatively simple or specialized for a network trained for a corresponding task, allowing the agent to plan and navigate with relative ease. However, in open-world scenarios, complex terrain and a variety of task types mean that the agent cannot smoothly execute tasks without analysis and decomposition. Therefore, in such situations, a Decomposer with task analysis and decomposition capabilities is highly necessary. As the process of analysis and decomposition requires the Decomposer to have strong understanding and logical abilities, we use the Large Language Model (GPT-4) as the core component of our Decomposer.

% We analyze and decompose tasks from top to bottom, and each subtask form includes all the information needed to complete the task (including subtask name, required quantity, materials needed for production and their quantities, tools required for production, and distribution description). When all subtasks are decomposed, we merge the same basic tasks into the earliest position of each basic task category (as shown in the figure, i.e., the basic task node with the greatest depth). The so-called basic tasks are subtasks that cannot be further decomposed.

% Once the above content is completed, we will pass the subtask information to the Planner for execution in a bottom-up order. This ensures that all subtasks have sufficient materials and tools before proceeding, preventing the cost of backtracking due to subtask failure caused by inadequate preparation.

% \subsection{Perceptor}
% The design of the Perceptor is of paramount importance in meeting the requirements of open-ended tasks in an open world. The Perceptor needs not only to understand different task demands to further actively perceive corresponding environmental information, but also to continuously interact with the Planner and provide relevant information until the Planner's planning conditions are met. To satisfy these capabilities, we chose a multimodal large language model as the core component of our Perceptor and set natural language dialogue as the medium for interaction between the Perceptor and the Planner. It is well known that a well-trained multimodal large language model not only has open-ended perception capabilities, but also the ability to interact continuously.

% To obtain such a model, we first constructed an instruction tuning dataset on the open-world platform of Minecraft. Based on the constructed dataset, we fine-tuned the existing multimodal large model. It's worth noting that, in order for the multimodal large model to better perceive Minecraft image data, we replaced the vision encoder in the multimodal large model with the vision encoder from MineClip, which has been pre-trained on a large amount of Minecraft image-text data. This modification produced desirable results.

% \textbf{Multimodal Instruction Data.} This dataset contains 50K image data collected on the MineDojo simulation platform. The image data covers nearly all content in Minecraft, including various ecological environments, various biological communities, various brightness intensities, underwater environments, etc., to ensure the model's capability to perceive the open world. Based on this, we collected, selected, and processed perceptual information corresponding to image data from the internal data of MineDojo (including blocks in the field of view, creatures, weather, occupation situations near the agent, etc.). Notably, we specially processed and filtered perspective information, leaving only information that can be obtained visually. We then constructed image-text question-and-answer pairs based on the images and perceptual information. To not limit the text interaction mode between the Perceptor and the Planner and to make the interaction more flexible and robust, we designed single-turn and multi-turn dialogue templates. We designed multiple question and answer forms for each perceptual information (200K instruction data pairs in total), thereby greatly reducing the probability of interaction failure between the Perceptor and the Planner. We plan to open-source all multimodal instruction data, hoping that this dataset can facilitate other works and promote the development of the community. Please refer to the appendix material for details on the dataset and data format.

% \subsection{Planner}
% We used the large language model (GPT-4) as our Planner. To better utilize the decision-making ability of large language models in open scenarios, we designed an active perception module that can continuously judge whether the information is sufficient to complete the current task and interact with the Perceptor continuously. We replaced the atomic action set with a purposeful workflow, improved the efficiency of completing similar tasks based on the external memory reference mechanism, and implemented a self-feedback mechanism based on failure cases.

% \textbf{Active Perception Module.} We specially designed corresponding prompt templates to implement the continuous interaction process between the Planner and the Perceptor. The Planner will continuously assess whether the currently collected information is sufficient to complete the corresponding task and continue to request missing information from the Perceptor in a question-and-answer format until it judges that there is enough information to complete the current task. It will then integrate all the acquired perception information into the final data used for decision-making. (Refer to the prompt diagram)

% \textbf{Workflow.} The large language model has strong logical reasoning ability, but atomic actions (such as moving forward one step, hitting once) often have no clear meaning and purpose. If atomic actions are used as the executable sequence, it will result in excessively long sequences leading to an exponential increase in trial and error costs. It may also cause delusions where the large language model cannot accurately understand the meaning of atomic actions and match the executable sequence with the current task. To solve this problem, we designed a purposeful workflow composed of atomic actions (refer to the table), which fully utilizes the reasoning ability of the large language model while greatly reducing the cost of trial and error, making the success rate of some long-term tasks significantly improved. Notably, we designed a language feedback workflow that can interact with people to provide real-time feedback during task execution, such as the following two situations (see table, two examples).


% \textbf{Reference Mechanism.} To reduce the Planner's repeated decisions on the same task and improve the decision efficiency of similar tasks, we proposed a reference mechanism. Whenever the Planner completes a new task, we will store its subtask name and workflow sequence in external memory. Whenever the Planner makes a decision, we will find the subtask most similar to the current one from the external memory and add its workflow sequence to the final data used for decision-making as a reference. (Refer to the prompt diagram)

% \textbf{Self-Feedback Mechanism.} Subtask execution failure is a common occurrence, and the Planner often needs multiple decisions to obtain a correct workflow sequence. To allow the Planner to gain experience from erroneous decisions and thus directionally correct the workflow sequence, we designed a self-feedback mechanism. The Planner will summarize and reflect on each execution error in the workflow and add this content to the final data used for decision-making in the new round. (Refer to the prompt diagram)




==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
